A probabilistic analysis on general probabilistic scheduling problems

The scheduling problem is a key class of optimization problems and has various kinds of applications both in practical and theoretical scenarios. In the scheduling problem, probabilistic analysis is a basic tool for investigating performance of scheduling algorithms, and therefore has been carried out by plenty amount of prior works. However, probabilistic analysis has several potential problems. For example, current research interest in the scheduling problem is limited to i.i.d. scenarios, due to its simplicity for analysis. This paper provides a new framework for probabilistic analysis in the scheduling problem and aims to deal with such problems. As a consequence, we obtain several theorems including a theoretical limit of the scheduling problem which can be applied to \emph{general, non-i.i.d. probability distributions}. Several information theoretic techniques, such as \emph{information-spectrum method}, turned out to be useful to prove our results. Since the scheduling problem has relations to many other research fields, our framework hopefully yields other interesting applications in the future.

==> Introduction.tex <==
\section{Introduction}
\subsection{Background}\label{Sec_Back}
\paragraph{Scheduling problems}
The scheduling problem  is a class of optimization problems which aims at assigning jobs (also called tasks) to machines 
in a time efficient way that minimizes the completion time (also called the makespan) of all the jobs.
In this paper we specifically focus on \emph{identical-machines scheduling}~\cite{McN59} (also called \emph{identical parallel machine scheduling}), 
which is one of the most well-investigated problem setting among many variants of scheduling problem.
In identical-machines scheduling problem, there are $m$ identical machines, and a job $j \in J$ takes processing time $p_j$ on any machine, i.e., the processing time is independent of a choice of machines.
\par
Identical-machines scheduling problem has so many applications in various kinds of practical scenarios and in theoretical computer science.
In practice, this scheduling problem has been emerged in many fields such as production lines, university, hospitals, and computer systems~(see \cite{CS90, Mok01} for good surveys).
On the other hand, in theoretical computer science this problem is known as an NP-hard problem~\cite{Kar72, GJ78, Har82} 
and therefore has been paid so much attention, often examined by approximating the optimal solution~\cite{Gra66, Gra69, HS87, AAWY98, GG19}.
Due to the practical importance as well as its relations to many other computational problems, 
identical-machines scheduling problem has become one of the core branches in several research fields, 
including operations research and computer science.

\paragraph{Probabilistic analysis}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Today, there are many algorithms~(often called as~\emph{heuristics} or \emph{policies}) for scheduling problem.
The list scheduling (LS) algorithm and the largest processing time (LPT) algorithm are two of the well-known algorithms.
In such cases, to select an appropriate scheduling algorithm for one's purpose, the one need to evaluate each algorithm with an appropriately chosen measure of performance.
One such candidate of the measure is the worst-case performance evaluation: For an scheduling algorithm $A$, the worst-case performance of the algorithm $A$ is given by $\WORST(A):=\max_{j^n \in J^n} A(j^n)$ where $A(j^n)$ denotes the makespan of the algorithm with input $j^n = (j_1, \ldots, j_n)$, which is a list of $n$ jobs.
This measure of performance gives a theoretical guarantee that any scheduling instance of the algorithm $A$ always has the makespan less than (or equal to) the quantity $\WORST(A)$.
This is one benefit of the worst-case analysis.
However the worst-case analysis has the crucial weak point: The makespan $A(j^n)$ of an input $j^n$ is often significantly shorter than the value $\WORST(A)$.
In other words, the hardest list of jobs:~$j^n_\mathrm{HARD} := \argmax A(j^n)$ may be really unlikely to happen in practice.
Today, there are several other measures of performance applied to scheduling algorithm, to overcome the weak point of the worst-case analysis.
\par
The average-case analysis, which is the other well-known method of the evaluation, can deal with the weak point of the worst-case analysis.
In the average-case analysis, a distribution $\Pr_{J^n}$ on $J^n$ is defined appropriately in order to reflect a practical situation, 
and performance of an algorithm $A$ is given as the expectation $\AVE(A, \Pr_{J^n}) := \E_{j^n \sim J^n}[A(j^n)]$ under the distribution $\Pr_{J^n}$.
As is easily seen, this analysis overcomes the weak point of the worst-case analysis, since jobs which occur with small probability affect the value $\AVE(A, \Pr_{J^n})$ not so much, even if makespans of the jobs are really large.
Therefore, the average-case analysis is usually more appropriate for practical situations and has been paid attention in scheduling problem.
\par
As mentioned above, the average-case analysis has been paid attention over decades, 
and therefore there is a certain number of works that analyze average-case behaviors of scheduling algorithms~(for example, \cite{PR96, CCG+00, CFGK91, CJLS93, CFW96, BBC18, BCEH21}), 
including analysis on an optimal algorithm that always outputs an optimal schedule having the shortest makespan.
 References~\cite{Kno81, Lue82, CFGK91, CCG+02, PR96} treat the average-case behaviors of \emph{optimal algorithms} for identical-machines scheduling problem or related problems.
For example, 
Ref.~\cite{PR96} characterized the constant $\theta := \lim_{n \to \infty}\E[\mathrm{OPT}_n(j^n)]/n$ when a list of jobs $j^n$ is $n$-i.i.d. distributed where $\mathrm{OPT}_n$ denotes an optimal algorithm.
On the other hand, some prior works such as References~\cite{FK87, CJLS93, CFW96, Li99, BCEH21} treat the average-case behaviors of several \emph{practical algorithms}.
In the case of practical algorithms, 
for example, 
Ref.~\cite{FK87} showed that the LPT algorithm asymptotically becomes the optimal one. 
That is, the makespan by the LPT algorithm (almost surely) converges to that of the optimal algorithm as $n \to \infty$, when a list of jobs $j^n$ is $n$-i.i.d. distributed.
For recent results on the LPT algorithm, see~Ref.~\cite{BCEH21} for example.
For its practical importance as well as theoretical interests, the average-case analysis on scheduling problem has been investigated in many prior works.
\par
Considering the usefulness of the average-case analysis, it may seem that the average-case analysis is the best way to evaluate performance of scheduling algorithms, and has no weak point at all.
However, the average-case analysis has at least two following problems.
First, in contrast to the worst-case analysis, the expectation $\E_{j^n \sim J^n}[A(j^n)]$ does not guarantee the worst-case performance of an algorithm $A$. 
This means, the makespan $A(j^n)$ of some jobs $j^n$ may become really long even if the average $\E_{j^n \sim J^n}[A(j^n)]$ is small.
Second, the average-case analysis usually need to assume i.i.d. conditions on distributions $\Pr_{J^n}$, which should reflect a practical situation appropriately.
Indeed, all the previous works assume the i.i.d. conditions. However, in practice this is too restrictive; 
there are many practical situations where distributions of jobs are correlated.
For example, jobs may form a Markov chain in some practical situations.
These are the two problems of the average-case analysis, and 
one of our main focus in this paper is to deal with the two above problems by appropriately re-defining a measure of performance.

\subsection{Our contributions}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
As mentioned in Section~\ref{Sec_Back}, both the worst-case and the average-case analysis have several problems when applied for evaluation of practical performances.
To avoid these problems, in this paper we introduce a new measure of performance, which is suitably defined to evaluate practical performance appropriately.
In short, our new measure discards a set $S_n$ of jobs that are \emph{unlikely to occur},
and evaluates the worst-case performance over the set $S^c_n$ of jobs which are likely to occur.
Formally, the new measure is defined as follows.
\begin{Def}
Let $S_n \subseteq J^n$ be a set of jobs unlikely to occur, i.e., $\Pr(S_n)$ is close to zero.
For a scheduling algorithm $\phi_n$ on $J^n$,
the new measure $\COST(\phi_n, S_n)$ is defined as
\begin{equation*}
\COST(\phi_n, S_n)
= \max_{j^n \in S_n} \phi_n(j^n)
\end{equation*}
where $\phi_n(j^n)$ is the makespan by the algorithm $\phi_n$ with an input $j^n$.
\end{Def}
This measure indeed captures the worst-case performance in a practical scenario,
while the average-case analysis fails to do so, as described in Section~\ref{Sec_Back}.
To see this, consider a scenario where a scheduling algorithm $\phi_n$ processes an input $j^n \in J^n$ only when the input belongs to the set $S_n$; otherwise the jobs $j^n$ are discarded and not scheduled to machines.
In this scenario, the value $\COST(\phi_n, S_n)$ obviously corresponds to the worst-case makespan produced by the algorithm $\phi_n$.
In our main contributions, Theorem~\ref{Thm_non-iid} and Theorem~\ref{Thm_Sec-order}, we successfully analyze fundamental behaviors of this new measure of performance.

\par
\subsubsection{First result} 
In our first result, we evaluate the limit: $\limsup_{n \to \infty} \frac{1}{n}\COST(\phi_n, S_n)$ for efficient algorithms\footnote{We often simply call a pair $(\phi_n, S_n)$ as an \emph{algorithm}.} $(\phi_n, S_n)$ 
whose discarding probability asymptotically vanishes, i.e.,  $\Pr_{J^n}(S_n^c) \to 0$ as $n \to \infty$.
More precisely, in our first result we evaluate the smallest possible value of $\limsup_{n \to \infty} \frac{1}{n}\COST(\phi_n, S_n)$ when $\Pr_{J^n}(S_n)$ must satisfy $\Pr_{J^n}(S_n) \to 1$.
To state the result formally, we introduce the notion of \emph{rate} as follows:
\begin{Def}
The rate $R > 0$ is achievable if and only if there is  a (sequence of) scheduling algorithm(s): $\{(\phi_n, S_n)\}_n$
such that $\lim_{n \to \infty} \Pr_{J^n}(S^c_n) = 0$ and $\limsup_{n \to \infty}\frac{1}{n}\COST(\phi_n, S_n) \leq R$ holds.
\end{Def}
Our goal is then to evaluate the infimum of the achievable rate: 
$\inf\{R > 0 \mid \text{The rate $R$ is achievable.} \}$,
and our first result characterizes this quantity as follows:
\begin{Thm}\label{Thm_non-iid}
For any $m$-identical machines scheduling problem, 
$\inf\{R > 0 \mid \text{The rate $R$ is achievable.} \} = \bar{E}$ holds
where
$\bar{E} := \inf\{\alpha \geq 0 \mid \lim_{n \to \infty} P_{\mathcal{J}^n}\{j^n \mid \frac{1}{n \cdot m} \sum_{i \leq n}T(j_i) > \alpha\} = 0\}$
and $T(j_i)$ denotes the processing time of a job $j_i$.
\end{Thm}
Let us mention several remarks regarding Theorem~\ref{Thm_non-iid}.
First and foremost, Theorem~\ref{Thm_non-iid} assumes almost nothing,  and thus can be applied to any scheduling problem with any kind of distribution.
In particular, we can apply Theorem~\ref{Thm_non-iid} to scheduling problems with non-i.i.d. distributions such as Markov processes, ergodic processes.
In the case of Markov processes, for example, the value $\bar{E}$ turns out to be equal to $\frac{1}{m}\E_J[T(J)]$ where $\E_J[T(J)]$ denotes the expectation of the processing time $T(J)$ with respect to its stationary distribution.
Second, considering that the discarding probability $\Pr_{J^n}(S^c_n)$ must need to vanish asymptotically, 
one may expect that there is asymptotically no difference between the worst-case measure $\frac{1}{n}\WORST[\mathrm{OPT}_n]$ and our evaluation $\bar{E}$.
However, this is not true. Even in a simple i.i.d. scenario, we see that $\frac{1}{n}\WORST[\mathrm{OPT}_n] \to \frac{1}{m}T_{\mathrm{max}}$ where $T_\mathrm{max} := \max_j T(j)$, but $\bar{E} = \frac{1}{m}\E[T(J)]$.
This means that there is a certain amount of savings by admitting the negligible probability of discarding.
Lastly, for several important cases such as i.i.d. scenarios, the quantity $\bar{E}$ and the average case evaluation $\lim_{n \to \infty} \E_J[\mathrm{OPT}_n(J)]/n$ coincide.
\begin{comment}
Our first result shows the theoretical limit of $\COST(\phi_n, S_n)$ when $n$ goes to $\infty$.
In contrast to prior works, in our first result 
there is no assumption on distributions $\{\Pr_{J^n}\}$, i.e., the distribution $\Pr_{J^n}$ does not need to be an i.i.d. distribution.
The formal statement of the first result is as follows.
\begin{Thm}\label{Thm_non-iid}
For any $S_n$ satisfying $\Pr_{J^n}(S_n) \to 1$ as $n \to \infty$ and any scheduling algorithm $\phi_n$, 
\begin{equation*}
\limsup_{n \to \infty} \frac{1}{n}\COST(\phi_n, S_n)
\geq \bar{E}
\end{equation*}
where
$\bar{E} := \inf\{\alpha \geq 0 \mid \lim_{n \to \infty} P_{\mathcal{J}^n}\{j^n \mid \frac{1}{n \cdot m} \sum_{i \leq n}T(j_i) > \alpha\} = 0\}$
and $T(j_i)$ denotes the processing time of a job $j_i$.
Moreover, this is tight: There is a sequence $\{(\phi_n, S_n)\}$ such that
\begin{equation*}
\limsup_{n \to \infty} \frac{1}{n}\COST(\phi_n, S_n)
\leq \bar{E}
\end{equation*}
holds.
\end{Thm}
For example, in the case of i.i.d. distributions, $\bar{E} = \frac{1}{m}\E_J[T(J)]$ holds.
\end{comment}
\subsubsection{Second result}

Even though our first result successfully characterizes the asymptotic rate of any scheduling problem with any distribution of jobs,
the result only gives the optimal rate in the asymptotic setting.
Needless to say, there are many practical situations where one may want to estimate the optimal value of $\COST(\phi_n, S_n)$ for finite number of jobs, e.g., $n = 1000$.
To deal with this problem, in our second result, we employ more precise analysis on the value $\COST(\phi^\OPT_n, S^\OPT_n)$ 
where $(\phi_n^\OPT, S_n^\OPT)$ is an optimal scheduling (with discarding probability $\varepsilon$) defined as $(\phi_n^\OPT, S_n^\OPT) = \argmin_{\Pr(S^c_n) \leq \varepsilon} \COST(\phi_n, S_n)$,
and characterize this value accurately for any finite $n$, up to an additive constant factor.
Our second result can be applied to any kind of i.i.d. scheduling problem.
The formal statement of our second result is as follows.
\begin{Thm}\label{Thm_Sec-order}
For any i.i.d. scheduling problem, 
\begin{equation*}
\COST(\phi^\textrm{opt}_n, S^\textrm{opt}_n) = \BARE \cdot n - \sqrt{n V(T(J)/m)}\Phi^{-1}(\varepsilon) + \Theta(1)
\end{equation*}
holds where $\Phi(x)$ is the standard Gaussian distribution and $V(T(J)/m) := \frac{1}{m^2}\E_J[(T(J) - \E[T(J)])^2]$.
\end{Thm}


\begin{comment}
In our second result, we consider the i.i.d. scenario and characterize the optimal performance without taking the limit $\limsup_{n \to \infty}$.
That is, 
\begin{Thm}\label{Thm_Sec-order}
Let $\Pr_{J^n}$ be an i.i.d. distribution on $J^n$.
Suppose $(\phi_n^\textrm{opt}, S_n^\textrm{opt})$ is an optimal scheduling among all schedulings $(\phi_n, S_n)$ satisfying $\Pr(S_n) \leq \varepsilon$. Then, 
\begin{equation*}
\COST(\phi^\textrm{opt}_n, S^\textrm{opt}_n) = \BARE \cdot n - \sqrt{n V(T(J)/m)}\Phi^{-1}(\varepsilon) + \Theta(1)
\end{equation*}
holds where $\Phi(x)$ is the standard Gaussian distribution and $V(T(J)/m) := \frac{1}{m^2}\E_J[(T(J) - \E[T(J)])^2]$.
\end{Thm}
\end{comment}

